Coverability: Realizability Lower Bounds

We introduce the problem of temporal coverability for realizability and synthesis. Namely, given a language of words that must be covered by a produced system, how to automatically produce such a system. We consider the case of coverability with no further specifications, where we have to show that the nondeterminism of the produced system is sufficient to produce all the words required in the output language. We show a counting argument on a deterministic automaton representing the language to be covered that allows to produce such a system. We then turn to the case of coverability with additional specification and give a precondition for the existence of a system that produces all required words and at the same time produces only computations satisfying the additional correctness criterion. We combine our counting argument on the deterministic automaton for the language to be covered with a ranking on the deterministic B\"uchi automaton for the correctness criterion. One of the major issues with practical realizability is the interaction between environment assumptions and system guarantees. In many cases, synthesis produces systems that are vacuous and concentrate on forcing the environment to falsify its assumptions instead of fulfilling their guarantees. Coverability offers an alternative approach to tackle this problem.

==> background.tex <==
\section{Background}
\label{section:prelim}
\label{section:background}

%We give basic notations covering finite-state automata, trees,
%%tree automata,
%and realizability.

We consider finite or infinite sequences of symbols from some finite
alphabet $\Sigma$. 
Given a {\em word} $w$, an element in $\Sigma^* \cup \Sigma^\omega$,
we denote by $w_i$ the $i^{th}$ letter of the word $w$, and by
$w_{\geq i}$ the suffix of $w$ starting at $w_i$ hence
$w=w_{\geq 0}=w_0w_1w_2 \ldots$.
The {\em length} of $w$ is denoted by $|w|$ and is defined to be $\omega$ for
infinite words.

\noindent{\bf Finite Word Automata and Finite Transducers.}
A {\em nondeterministic finite word} automaton is 
$N=\langle\Sigma,S,\delta,s_0,F\rangle$, where $\Sigma$ is the finite 
alphabet, $S$ is the finite set of states,
$\delta:S\times \Sigma\rightarrow 2^S$ is the transition 
function,
$s_0\in S$ is the initial state, 
and $F$ is the acceptance set. 
We can run $N$ either on finite words
({\em nondeterministic finite word} automaton or {\em NFW} for short)
or on infinite words ({\em nondeterministic B\"uchi word} automaton or
{\em NBW} for short).
The automaton is {\em deterministic} if for every state $s\in S$ and
every letter $\sigma\in\Sigma$ we have $|\delta(s,\sigma)|\leq 1$.
Deterministic automata are denoted DFW and DBW, for short.

A {\em run} of $N$ on a finite word $w=w_0,...,w_l$
is a finite sequence of states
$t_0,t_1,\ldots,t_{l+1}\in S^+$ where $t_0=s_0$ and for every $0\leq i
\leq l$ we have $t_{i+1}\in \delta(t_i,w_i)$.
A run is {\em accepting} if $i_m=l+1$ and $t_m\in F$.
A {\em run} of $N$ on an infinite word $w=w_0,w_1,...$ is defined
similarly as an infinite sequence.
For an NBW, a run is
{\em accepting} if it visits $F$ infinitely often.

A word $w$ is {\em accepted} by $N$ if it has an accepting run over $w$. 
The {\em language} of $N$ is the set of words accepted by $N$, denoted
by $L(N)$.


A finite {\em transducer} $\cD$ is  
$\pair{\Psi,\Sigma,Q,\eta,q_0,L}$, where 
$\Psi$ is a finite set of directions, 
$\Sigma$ is a finite alphabet, 
$Q$ is a finite set of states, 
$\eta: Q \times \Psi \rightarrow Q$ is a partial transition
function, 
$q_0\in Q$ is a start state, 
and $L: Q \rightarrow \Sigma$ is a labeling function. 
When $\eta$ is defined for every $q\in Q$ and $\psi\in \Psi$ we 
say that $\cD$ is \emph{full}.
We define $\eta: \Psi^* \rightarrow Q$ in 
the standard way: $\eta(\varepsilon)=q_0$ and $\eta(x\psi)=\eta(\eta(x),\psi)$.
Similarly, we define the extended labeling 
$L:\Psi^*\rightarrow \Sigma^+$ by considering 
$L(\varepsilon)=L(q_0)$ and $L(x\psi)=L(x)\cdot L(\eta(x\psi))$.
Notice that, unless $\cD$ is full, $\eta$ and $L$ may be partial functions. 
Intuitively, a transducer is a labeled finite graph with 
a designated start node, where the edges are labeled by $\Psi$ and the
nodes are labeled by $\Sigma$.
The language of a transducer $\cD$ is the set 
$\{ L(x) ~|~ x\in \Psi^* \mbox{ and } L(x) \mbox{ defined}\}$. 
That is, all the possible words that label paths through the graph of $\cD$. 
A transducer $\cD$ is \emph{deterministic} if for every state $q\in Q$ and 
every two letters $\psi_1,\psi_2\in \Psi$ we have if 
$L(\eta(q,\psi_1))=L(\eta(q,\psi_2))$ then 
$\eta(q,\psi_1)=\eta(q,\psi_2)$.
That is, every state $q$ and for every letter $\sigma\in\Sigma$ there is 
at most one successor of $q$ labeled by $\Sigma$.
Given a nondeterministic transducer, it is possible to construct a 
deterministic transducer with the same language.
This is a simple variant of the determinization of NFW \cite{RS59}.

\noindent
{\bf Trees.}
Given a finite set $\Upsilon$ of directions, 
an {\em $\Upsilon$-tree} is a set $T \subseteq
\Upsilon^{*}$ such that if $x \cdot \upsilon \in T$, where 
$x \in \Upsilon^{*}$ and $\upsilon \in \Upsilon$,
then also $x \in T$. 
The elements of $T$ are called {\em nodes},
and the empty word $\varepsilon$ is the {\em root} of $T$.
For every $\upsilon \in \Upsilon$ and $x \in T$,
the node 
$x$ is the {\em parent\/} of $x \cdot \upsilon$.
Each node $x\in T$ has a {\em direction} in
$\Upsilon$.
We assume that the root has some fixed direction $\upsilon_0\in\Upsilon$.
The direction of a node $x \cdot \upsilon$ is $\upsilon$. 
We denote by $dir(x)$ the direction of node $x$. 
An $\Upsilon$-tree $T$ is a {\em full infinite tree} if
$T=\Upsilon^*$. 
Unless otherwise mentioned, we consider here full infinite trees. 
A {\em path} $\pi$ of a tree $T$ is a set $\pi \subseteq T$ such that
$\varepsilon \in \pi$ and for every $x \in \pi$ there exists a unique
$\upsilon \in \Upsilon$ such that $x \cdot \upsilon\in \pi$. 
For a node $x\in \Upsilon^*$ in the tree, we denote by $x|_i$ the
prefix of $x$ up to length $i$.
For example, $x|_0=\varepsilon$ and $x|_{|x|}=x$.

Given two sets $\Upsilon$ and $\Sigma$, a {\em $\Sigma$-labeled
$\Upsilon$-tree} is a pair $\pair{T,\tau}$ where $T$ is an $\Upsilon$-tree
and $\tau:T \rightarrow \Sigma$ maps each node of $T$ to a
letter in $\Sigma$.
%When $\Upsilon$ and $\Sigma$ are not important or
%clear from the context, we call $\pair{T,\tau}$ a labeled tree.
A $\Upsilon\times\Sigma$-labeled $\Upsilon$-tree $T=\pair{\Upsilon^*,\tau}$ 
is \emph{directed} if for every $x\upsilon\in\Upsilon^+$ we have 
$\tau(x) \in \{\upsilon\}\times\Sigma$ and
$\tau(\varepsilon)\in \{\upsilon_0\}\times \Sigma$. 
For a node $x\in\Upsilon^*$ the \emph{prefix-label} of $x$ is the finite 
word $w$ that labels the path from the root of the tree to $x$. 
More formally, $|w|=|x|+1$ and $w_i=\tau(x|_i)$.
We denote the prefix-label of $x$ by $\vec{\tau}(x)$.
We define the language of the tree $T$ to be $L(T) = \{\vec{\tau}(x)
~|~ x\in \Upsilon^*\}$.

A labeled tree is {\em regular} if it is the unwinding of some full transducer.
Formally, 
a $\Sigma$-labeled $\Upsilon$-tree $\pair{\Upsilon^*,\tau}$ is regular 
if there exists a full transducer $D=\pair{\Upsilon,\Sigma,Q,\eta,q_0,L}$,
such that for every $x\in \Upsilon^*$, we have $\tau(x)=L(x)$.
The size of 
$\pair{\Upsilon^*,\tau}$, denoted $\| \tau \|$, is $|Q|$,
the number of states of $\cD$. 

%{\em Alternating automata\/} on infinite trees generalize
%nondeterministic tree automata and were first introduced in \cite{MS87}.
%For a finite set $X$, let ${\cal B}^{+}(X)$ be the set of positive
%Boolean formulas over $X$ (i.e., boolean
%formulas built from elements in $X$ using $\wedge$ and $\vee$), where 
%we also allow the formulas $\true$ and $\false$,
%and, as usual, $\wedge$ has precedence over $\vee$.
%For a set $Y \subseteq X$ and a formula $\theta \in {\cal B}^{+}(X)$,
%we say that $Y$ {\em satisfies\/} $\theta$ (denoted $Y \models
%\theta$) iff assigning $\true$ to
%elements in $Y$ and assigning $\false$ to elements in $X \setminus Y$
%makes $\theta$ true.
%An {\em alternating automaton} over $\Sigma$-labeled
%$\Upsilon$-trees 
%is a tuple $A=\pair{\Sigma,Q,\delta,q_0,F}$, 
%where  $\Sigma$ is the input alphabet,  
%$Q$ is a finite set of states,
%$\delta : Q \times \Sigma \rightarrow 
%{\cal B}^{+}(\Upsilon \times Q)$ is the transition function,
%$q_{0} \in Q$ is an initial state,
%and $F$ is the acceptance condition.
%
%A run of an alternating automaton $A$ over a labeled
%tree $\pair{\Upsilon^*,\tau}$ is a
%labeled tree $\pair{T_r,r}$ in which every node is labeled by an 
%element of $\Upsilon^* \times Q$.   
%A node in $T_r$, labeled by $(x,q)$, describes a copy of the automaton
%that is in the state $q$ and reads the node $x$ of $\Upsilon^*$.
%Note that many nodes of $T_r$ can correspond to the same node of
%$\Upsilon^*$; 
%there is no one-to-one correspondence between the nodes of the run
%and the nodes of the input tree.
%The labels of a node and its successors have to satisfy the
%transition function.
%Formally, a run $\pair{T_r,r}$ is a $\Sigma_r$-labeled $\Gamma$-tree,
%for some set $\Gamma$ of directions,
%where $\Sigma_r=\Upsilon^* \times Q$ and $\pair{T_r,r}$ satisfies the
%following: 
%\begin{enumerate}
%\item
%$\varepsilon \in T_r$ and $r(\varepsilon)=(\varepsilon,q_0)$.
%\item
%Consider $y \in T_r$ with $r(y)=(x,q)$ and $\delta(q,\tau(x))=\theta$.
%Then there is a (possibly empty) set
%$S \subseteq \Upsilon \times Q$, such that 
%$S$ satisfies $\theta$, and
%for all $(\upsilon,q') \in S$, there is $\gamma \in \Gamma$ such that
%$y \cdot \gamma \in T_r$ and $r(y\cdot \gamma)=(x \cdot \upsilon,q')$.
%\end{enumerate}
%
%A run $\pair{T_r,r}$ is {\em accepting\/} if all its infinite paths 
%satisfy the acceptance condition. 
%We consider here {\em B\"uchi} and {\em parity\/} acceptance
%conditions \cite{Buc62,EJ91}. 
%A parity condition over a state set $Q$ is a finite sequence
%$F=\{F_1,F_2,\ldots,F_k\}$ of subsets of $Q$, where
%$F_1 \subseteq F_2 \subseteq \ldots \subseteq F_k=Q$.
%The number $k$ of sets is called the {\em index\/} of $A$.
%Given a run $\pair{T_r,r}$ and an infinite path
%$\pi \subseteq T_r$, let ${\it inf}(\pi) \subseteq Q$ be such that $q \in
%{\it inf}(\pi)$ if and only if there are infinitely many $y \in \pi$ for
%which $r(y) \in \Upsilon^* \times \{q\}$. That is, ${\it inf}(\pi)$ contains
%exactly all the states that appear infinitely often in $\pi$.
%A path $\pi$ satisfies the parity condition $F$ if there is an even
%$1 \leq i \leq k$ such that  ${\it inf}(\pi) \cap F_i \neq \emptyset$ and 
%${\it inf}(\pi) \cap F_{i-1} = \emptyset$.
%A B\"uchi acceptance condition consists of a set $F_2 \subseteq Q$ and
%it can be viewed as a special case of a parity condition of index 3,
%where $F = \{\emptyset, F_2, Q\}$. Thus, a run is
%accepting according to the B\"uchi condition $F_2$ if every path in
%the run visits $F_2$ infinitely often. 
%An automaton accepts a labeled tree if there exists a run 
%that accepts it.  
%We denote by ${\cal L}(A)$ the set of all $\Sigma$-labeled
%trees that $A$ accepts. The automaton $A$ is {\em nonempty\/} iff 
%${\cal L}(A) \neq \emptyset$.
%
%An automaton is  
%nondeterministic if in every transition exactly one copy of the
%automaton is sent in every direction in $\Upsilon$. 
%Formally, an automaton is nondeterministic if for every
%state $q\in Q$ and letter $\sigma \in \Sigma$ there exists some set
%$I$ such that $\delta(q,\sigma)= \bigvee_{i\in I} \bigwedge_{\upsilon
%\in \Upsilon} (s_{i,\upsilon},\upsilon)$.
%Equivalently, we can describe the transition function of a
%nondeterministic automaton as $\delta: Q \times \Sigma \rightarrow
%2^{(Q^{|\Upsilon|})}$. The tuple $\pair{q_1, \ldots, q_{|\Upsilon|}}
%\in \delta(q,\sigma)$ is equivalent to the disjunct $(q_1,\upsilon_1)
%\wedge \ldots \wedge (q_{|\Upsilon|},\upsilon_{|\Upsilon|})$.
%
%We use acronyms in
%$\{A,N,D\} \times \{P,B,F\} \times \{T,W\}$ to denote the different types
%of automata. The first symbol stands for the branching
%mode of the automaton: $A$ for alternating, $N$ for
%nondeterministic, and $D$ for deterministic. The second symbol stands
%for the type of acceptance used by the automaton: $P$ for parity, $B$
%for B\"uchi, and $F$ for finite.
%The last symbol stands for the object the automaton is reading: $T$ for
%trees and $W$ for words.
%For example, an APT is an alternating parity tree automaton and
%an NPT is a nondeterministic parity tree automaton.

\noindent
{\bf Realizability.}
Consider an NBW $N=\langle \Upsilon\times \Sigma, S,\delta, s_0, F\rangle$, where the
alphabet has the structure 
$\Upsilon\times \Sigma$ for some sets of \emph{inputs} and \emph{outputs} $\Upsilon$
and $\Sigma$, respectively.
The language of $N$ is \emph{realizable} if there exists a 
full directed $\Upsilon\times\Sigma$-labeled $\Upsilon$-tree $T$ such that
$L(T)\subseteq L(N)$. We say that $T$ \emph{realizes} $N$.
Notice that this implies that the initial state of $N$ reads the label
of the root of the tree.
As the direction of the root is $\upsilon_0$ this implies that for some
$\sigma\in\Sigma$ we have $\delta(s_0,(\upsilon_0,\sigma))\neq \emptyset$.

\begin{theorem}{\rm \cite{PR89a}}
The language of $N$ is realizable iff
there exists a finite transducer $D_N$ over directions $\Upsilon$
and alphabet $\Upsilon\times\Sigma$ such that for every 
$q\in Q$ and every $\upsilon\in\Upsilon$ we have
$L(\eta(q,\upsilon))\in \{\upsilon\}\times\Psi$ such that 
$L(D_N)\subseteq L(N)$.
\end{theorem}


==> buchi.tex <==
\section{Coverability with B\"uchi Realizability}
\label{section:buchi}

We extend the problem of coverability by considering simultaneously that
all the paths in the tree must be labeled by words accepted by a DBW.
We give a precondition for coverability that is not complete.

Consider a transducer $\cD=\pair{\Psi,\Sigma,Q,\eta,q_0,L}$ and a  
DBW $B=\pair{\Upsilon\times\Sigma,S,\delta,s_0,F}$.
As usual, in order to realize the DBW for every $\upsilon\in\Upsilon$
we have to choose 
a $\sigma\in\Sigma$ such that the infinite word resulting from such repeated 
interactions is in the language of $B$.
We note that initially one has to choose a $\sigma\in\Sigma$ only for
the initial direction $\upsilon_0$. 
For the transducer, $\cD$, we choose to ignore the input $\Upsilon$.
The reasoning is that the tree must include all possible options for
$\Upsilon$ and there is no choice about their inclusion.
In order to define covering in a way that does take the input into
account we would have to allow the transducer to ``choose'' between
different options for inputs and enforce a very unusual definition of
what is the language of the transducer.
The techniques we establish will form foundations for such definitions
of covering as well.

\begin{definition}{\rm Covering with B\"uchi Realizability.}
  The language of a transducer $\cD$ is coverable while realizing
  DBW $B$ with branching $\Upsilon$ if there is a full directed
  $\Upsilon\times\Sigma$-labeled 
  $\Upsilon$-tree that covers $\cD$ and realizes $B$. 
\end{definition} 

As before, the directions $\Psi$ read by $\cD$ are used to
distinguish between different transitions and do not appear on the
tree.

We note that if $L(\cD) \neg\subseteq L(B)$ then covering is clearly
impossible.
As $B$ is deterministic, the check whether $L(\cD)\subseteq L(B)$ is
easy to perform.
If the upper bound language is given as a nondeterministic automaton
then the very first step in checking coverability would be to check
language inclusion between $\cD$ and $B$.
Here, we assume that $L(\cD)\subseteq L(B)$ and consider a system that
can output all possible output symbols at every stage of its
computation.
Thus, the issue of language containment in the language of a
nondeterministic system is largely bypassed. 

Consider for example the transducer in Figure~\ref{figure:example 2}
again.
Let $\Upsilon=\{\alpha,\beta\}$ be the set of input letters.
We add a property that dictates that if a $b$ is combined with
direction $\beta$ then only $c$ can follow it and that $c$s must
follow a $b$ in direction $\alpha$ infinitely often (unless completely
diverging from the language of the transducer).
The safety part of this condition means that if a copy of state $q_1$
appears in direction $\beta$ it can't be followed by copies of states
$q_2$ and $q_3$.
This means that we want the copy of state $q_1$ in direction $\alpha$
to be followed by $q_2$ and $q_3$.
However, this conflicts with the liveness property telling us that
$q_1$ in direction $\alpha$ should be followed infinitely often by
$q_0$.
In order to accommodate this requirement we must include two copies of
$q_0$ with output $c$ in level 3 of the tree both of them having input
$\alpha$ followed by output $b$.
This is in contrast to the previous case where one copy of $q_0$ in
level 3 was sufficient.
In particular, the root of the tree, which corresponds to the initial
state $q_0$ of the transducer and the transition $(s_0,(.,c),s_1^a)$
of the DBW is covered in a different way from the nodes $\beta\alpha$
and $\beta\beta$, which also correspond to the initial state $q_0$ of
the transducer and the transition $(s_0,(.,c),s_1^a)$. 

%If for example we change the transducer in
%Figure~\ref{figure:example 2} by requiring that the $b$ output by
%state $q_3$ is followed by 
%all of $a$, $b$, and $c$ then simple covering is still possible but
%covering with the DBW above is impossible.
%This is for two reasons, first the $b$ output by $q_1$ would have to
%have one successor corresponding to $q_2$ ($a$), \emph{two} successors
%corresponding to $q_3$ ($b$) and one successor corresponding to $q_0$
%($c$).
%However, the three successors outputting $a$ and $b$ would have to
%follow direction $\alpha$, which is impossible and the successor
%outputting $c$ would never be able to follow a $b$ in direction
%$\alpha$ falsifying liveness.

\begin{figure}[bt]
  \begin{minipage}{0.5\textwidth}
    \input{figures/buchiaut1.tex}
  \end{minipage}
  \begin{minipage}{0.5\textwidth}
    \input{figures/ex2buchitree.tex}
  \end{minipage}
  \vspace*{-3mm}
  \caption{\label{figure:example buchi}
    A DBW enforcing that after a
    $(\beta,b)$ ($b$ in direction $\beta$) the outputs $a$ and $b$
    cannot appear and that a $c$ follows a $(\alpha,b)$ (a $b$ in
    direction $\alpha$) infinitely often
    and a tree covering the transducer in
    Figure~\ref{figure:example 2} and realizing this DBW.
    Directions that are missing from the tree are not restricted by
    the transducer and can be be easily completed in a way that
    realizes the DBW.
  }
  \vspace*{-6mm}
  \end{figure}

We now develop techniques similar to those developed in
Section~\ref{section:simple} for proving coverability.
As notations get quite cumbersome we start with a simpler definition
that shows only cover with no memory and extend it to cover with
memory later.

\subsection{Coverability without Memory}
\label{subsection:buchi memoryless}
Consider a transducer $\cD=\pair{\Psi,\Sigma,Q,\eta,q_0,L}$ and a  
DBW $B=\pair{\Upsilon\times\Sigma,S,\delta,s_0,F}$.
We assume that $q^\bot \notin Q$ and let $Q^\bot$ denote
$Q\cup \{q^\bot\}$.
A combined \emph{weight-ranking} for $B$ and $\cD$ is
$w:(Q\times S) \cup (Q\times S \times \Psi \times
\Upsilon) \rightarrow \mathbb{N}$ and
$d:Q^\bot \times S \rightarrow (\mathbb{N} \cup \{\infty\})$
such that the following conditions hold.
\begin{compactitem}
\item
  For the weight distribution $w$ we have the following:
  \begin{compactitem}
  \item
    $w(q_0,\delta(s_0,(\upsilon_0,L(q_0))))=1$.
  \item
    For every $q\in Q$, $s\in S$, $\psi \in \Psi$, and
    $\upsilon\in\Upsilon$ if $w(q,s,\psi,\upsilon>0$ then
    $\eta(q,\psi)$ is defined and
    $\delta(s,(\upsilon,L(\eta(q,\psi))))$ is defined.

    That is, weight can be associated only with real (combined)
    transitions of $\cD$ and $B$.
  \item
    For every $q \in Q$ and $s\in S$ we have 
    $|\Upsilon|\cdot w(q,s) \geq 
    \sum_{(\psi,\upsilon)}w(q,s,\psi,\upsilon)$.

    That is, the weight of $w(q,s)$ is sufficient to cover the weights
    of all outgoing transitions. 
  \item
    For every $q\in Q$, $s\in S$, and $\upsilon \in \Upsilon$
    we have $\sum_{\psi\in\Psi} w(q,s,\psi,\upsilon) \leq w(q,s)$.

    That is, we can use at most $w(q,s)$ successors in direction
    $\upsilon$. 
  \item
    For every $q\in Q$, $s\in S$, $\psi\in\Psi$, and $\upsilon
    \in \Upsilon$ we have $w(q,s,\psi,\upsilon) \geq
    w(\eta(q,\psi),\delta(s,(\upsilon,L(\eta(q,\psi)))))$.

    That is, the weight of a transition is sufficient to cover the
    target of that transition.
  \end{compactitem}
\item
  For the ranking $d$ we have the following:
  \begin{compactitem}
  \item
    $d(q_0,\delta(s_0,\upsilon_0,L(q_0)))\neq \infty$

    That is, the state reached after $q_0$ reads the direction of the
    root and the label of $q_0$ has a finite rank. 
  \item
    For every $s\notin B$ and for every $q\in Q$ and
    $\upsilon \in \Upsilon$ such that $d(s,q)\neq \infty$: 
    \begin{compactitem}
    \item
      For every $\psi\in\Psi$
      such that $w(q,s,\psi,\upsilon) >0$ we have 
      $d(q,s) >
      d(\eta(q,\psi),\delta(s,(\upsilon,L(\eta(q,\psi)))))$.
    \item
      If $\sum_{\psi\in\Psi}w(q,s,\psi,\upsilon)<w(q,s)$ then there
      is some $\sigma\in\Sigma$ such that
      $d(q,s) > d(q^\bot,\delta(s,(\upsilon,\sigma)))$.
    \end{compactitem}

    That is, if $s$ is not a B\"uchi state then the rank must decrease
    in all directions of the tree. Either by continuing to cover the
    transducer or by considering only realizability. 
  \item
    For every $s\in B$ and for every $q\in Q$
    and $\upsilon\in\Upsilon$ such that $d(s,q)\neq \infty$:
    \begin{compactitem}
    \item
      For every $\psi\in\Psi$ such that
      $w(q,s,\psi,\upsilon)>0$ we have
      $d(\eta(q,\psi),\delta(s,(\upsilon,L(\eta(q,\psi)))))\neq
      \infty$.
    \item
      If $\sum_{\psi\in\Psi}w(q,s,\psi,\upsilon)<w(q,s)$ then there is
      some 
      $\sigma\in\Sigma$ such that
      $d(q^\bot,\delta(s,(\upsilon,\sigma))) \neq \infty$.
    \end{compactitem}

    That is, if $s$ is a B\"uchi state then the rank must be finite in
    all directions of the tree. Either by continuing to cover the
    transducer or by considering only realizability. 
  \item
    If for some $s\in S$ we have $d(q^\bot,s)\neq \infty$
    then:
    \begin{compactitem}
    \item
      If $s\notin B$ then for every $\upsilon\in\Upsilon$ there is
      some $\sigma\in\Sigma$ such that
      $d(q^\bot,s)>d(q^\bot,\delta(s,(\upsilon,\sigma)))$.
    \item
      If $s\in B$ then for every $\upsilon\in\Upsilon$ there is some
      $\sigma\in\Sigma$ such that
      $d(q^\bot,\delta(s,(\upsilon,\sigma)))\neq \infty$. 
    \end{compactitem}
    That is, in order to ensure realizability the ranking must be
    decreasing for non-B\"uchi states and defined for successors of
    B\"uchi states. 
  \end{compactitem}
\end{compactitem}
  
This definition combines the weight with a B\"uchi ranking, where the
weight shows that the language of $\cD$ is coverable and the
ranking shows that the language of the tree realizes the language of $B$.
The intuition is similar to that of the weight of the simple covering.
With $w(q,s)$ nodes in the tree we can cover the language of
$\cD_q$ realizing the language of $B_s$.
The ranking $d$ ensures that at the same time the language of $B$ is
realizable.
When the covering does not constrain the whole tree then the ranking
with the ``state'' $q^\bot$ ensures that the language of $B$ is
realizable without caring about the weights.

\begin{theorem}
  If there is a combined weight-ranking
  $w$ and $d$ for $B$ and $\cD$ then
  the language of $\cD$ is coverable while realizing
  $B$ with branching $\Upsilon$ 
\label{theorem:buchi memoryless coverability}
\end{theorem}

\begin{proof}
Suppose that there is a combined weight-ranking $w$ and $d$ for $B$
and $\cD$.

Given a run $r_q=q_0,q_1,\ldots,q_n$ of $\cD$ and a run
$r_s=s_0,s_1,\ldots, s_{n+1}$ of $B$ we denote by $r_q \otimes r_s\in
(Q\times S)^+$ the \emph{joint run} $(q_0,s_1),\ldots (q_n,s_{n+1})$
(notice the omission of $s_0$). 
We are going to use joint runs to label the nodes of $\Upsilon^*$.
We also consider extensions of runs of $\cD$ of the form
$q_0,q_1,\ldots, q_n,q^\bot,\ldots,q^\bot$, where $q_0,q_1,\ldots,
q_n$ is a run of $\cD$ and it is extended by a number of
``visits'' to $q^\bot$.

Consider the tree $\Upsilon^*$.
Based on the weight distribution $w$ and the ranking $d$ we construct
a $(Q^\bot \times S)^+$-labeled $\Upsilon$-tree
$T=\pair{\Upsilon^*,\pi}$ by induction.
The labeling maintains the following invariants:
\begin{itemize}
\item
  for every $x\in \Upsilon^*$ we have $|x|+1=|\pi(x)|$.
\item
  consider a run $r_q$ of $\cD$ ending in state $q\neq q^\bot$
  such that for some run $r_s$ of 
  $B$ ending in state $s$ there is a node $x\in \Upsilon^*$ labeled by
  $r_q \otimes r_s$, i.e., $\pi(x)=r_q\otimes r_s$. 
  Then, there are at least $w(q,s)$ nodes $\{x_1,\ldots,x_{w(q,s)}\}$
  in $\Upsilon^*$ such that for every $i$ there is some run $r^i_s$
  of $B$ ending in $s$ such that $\pi(x_i)=r_q\otimes r^i_{s}$.

  That is, $r_q$ is complemented by runs $r_s$ of $B$ so that there
  are $w(q,s)$ copies of $r_q$ in $T$.
\item
  for every $x\upsilon\in\Upsilon^+$ if
  $\pi(x\upsilon)=r(q,s)(q',s')$ then $\pi(x)=r(q,s)$ for some $q'$
  and $s'$ such that either $(q,\psi,q')\in \eta$ and
  $(s,(\upsilon,L(q)),s') \in \delta$ or
  $q'=q^\bot$ and for some $\sigma\in\Sigma$ we have
  $(s,(\upsilon,\sigma),s') \in \delta$. 

  That is, the nodes in the tree are effectively labeled by runs of
  $\cD$ and $B$ and children of nodes are labeled by runs that
  extend the run labeling their parent.
\end{itemize}

We set $\pi(\varepsilon)=(q_0,\delta(s_0,(\upsilon_0,L(q_0))))$.
Clearly, $|\varepsilon|+1=|(q_0,\delta(s_0,(\upsilon_0,L(q_0))))|$.
By definition of weight 
$w(q_0,\delta(s_0,(\upsilon_0,L(q_0))))=1$ and hence one node
$\varepsilon$ labeled by the joint run
$(q_0,\delta(s_0,(\upsilon_0,L(q_0))))$ is sufficient.

Consider a run $r_q$ of $\cD$ ending in state $q\neq q^\bot$ and
a state $s$ of $B$.
Let 
$X=\{x_1,\ldots, x_{w(q,s)}\}\subset \Upsilon^*$ be such  
that for every $i$ there is some run $r_s^i$ of $B$ ending in $s$ and
$\pi(x_i)=r_q\otimes r_s^i$.
By definition of the weight distribution we have 
$|\Upsilon|\cdot w(q,s) \geq \sum_{(q,s,\psi,\upsilon)}
w(q,s,\psi,\upsilon)$.
Let $Y$ denote the set of nodes 
$\{x\cdot \upsilon ~|~ x\in X \mbox{ and } \upsilon \in \Upsilon\}$.
It follows that $|Y|=|\Upsilon|\times w(q,s)$.

Furthermore, for every $\upsilon\in\Upsilon$ we have
(i) $\sum_{\psi\in\Psi}w(q,s,\psi,\upsilon) \leq w(q,s)$ and
(ii) 
$w(q,s,\psi,\upsilon)\geq
w(\eta(q,\psi),\delta(s,(\upsilon,L(\eta(q,\psi)))))$.
It follows that we can partition $Y$ such that for every
$(q,s,\psi,\upsilon)$ there is a set  
$Y_{(q,s,\psi,\upsilon)}$ of size $w(q,s,\psi,\upsilon)$
such that $Y_{(q,s,\psi,\upsilon)}\subseteq X\cdot \{\upsilon\}$ and for every two
$(q,s,\psi,\upsilon)$ and $(q,s,\psi',\upsilon')$ such that either
$\psi\neq \psi'$ or $\upsilon\neq \upsilon'$ 
we have 
$Y_{(q,s,\psi,\upsilon)}\cap Y_{(q,s,\psi',\upsilon')}=\emptyset$.
Let $\overline{Y}$ denote the set of nodes in $Y$ that are 
not included in the subsets $Y_{(q,s,\psi,\upsilon)}$.
That is,
$$\overline{Y}=Y\setminus (\bigcup_{(q,s,\psi,\upsilon)}Y_{(q,s,\psi,\upsilon)}).$$

It follows that it is safe to label the nodes $x\upsilon\in
Y_{(q,s,\psi,\upsilon)}$ by the combined run $\pi(x)\cdot
(\eta(q,\psi),\delta(s,(\upsilon,L(\eta(q,\psi)))))$.
That is, for $x\upsilon\in Y_{(q,s,\psi,\upsilon)}$ we set
$\pi(x\upsilon)=\pi(x)\cdot (\eta(q,\psi),\delta(s,(\upsilon,L(\eta(q,\psi)))))$.

Consider a node $x\upsilon\in \overline{Y}$.
From it being in $\overline{Y}$, it follows
that $\sum_{\psi\in\Psi}w(q,s,\psi,\upsilon)<w(q,s)$.
Hence, for some $\sigma\in\Sigma$ we know that
$d(q^\bot,\delta(s,(\upsilon,\sigma)))$ is not $\infty$ and if needed
is smaller than $d(q,s)$.
We label the node $x\upsilon$ by the combined run $\pi(x)\cdot
(q^\bot,\delta(\upsilon,\sigma))$.
That is, for $x\upsilon\in\overline{Y}$ we set
$\pi(x\upsilon)=\pi(x)\cdot (q^\bot,\delta(\upsilon,\sigma))$.

There are at least  
$w(\eta(q,\psi),\delta(s,(\upsilon,\eta(q,\psi))))$ nodes labeled 
by $r\cdot (\eta(q,\psi),\delta(s,(\upsilon,\eta(q,\psi))))$.  
As $|x|+1=|r|$ then $|x\upsilon|+1=|r\cdot
(\eta(q,\psi),\delta(s,(\upsilon,\eta(q,\psi))))|$. 
Finally, $\pi(x\upsilon)$ extends $\pi(x)$ by
$(\eta(q,\psi),\delta(s,(\upsilon,\eta(q,\psi))))$.  

If the run $r_{q^\bot}$ of $\cD$ ends in $q^\bot$ then by the
definition of $d$ for every $\upsilon\in\Upsilon$ there is some
$\sigma_\upsilon\in\Sigma$ such that
$d(q^\bot,\delta(s,(\upsilon,\sigma_\upsilon)))$ is 
not $\infty$ and if needed is smaller than $d(q^\bot,s)$.
We label the node $x\upsilon$ by
$\pi(x)\cdot(q^\bot,\delta(s,(\upsilon,\sigma_\upsilon)))$.
That is,
$\pi(x\upsilon)=\pi(x)\cdot(q^\bot,\delta(s,(\upsilon,\sigma_\upsilon)))$.

This completes the construction of $\pi$ by induction.
% option to shorten here - the rest of the argument can be moved to
% appendix. 
We now use $\pi$ to show a labeling $\tau$ for $\Upsilon^*$ that
covers the language of $\cD$ and realizes the language of $B$.
By the invariant for labeling, for every run $r_1$ of $\cD$ there
is (at least) a  
node $x\in \Upsilon^*$ such that $\pi(x)=r_1\otimes r_2$ for some run
$r_2$ of $B$.
We set $\tau(x)=L(q)$, where $q$ is the last state of
$r_1$.
We see that $L(\cD)\subseteq L(T)$ as required.

Also, by the properties of $d$ it follows that every run of $B$ visits
its acceptance set infinitely often. This shows that every path in the
tree is accepted by $B$.
\end{proof}

\begin{corollary}
  In a (memoryless) combined weight-ranking for $B$ and $\cD$ and branching
  $\Upsilon$ all weights are bounded by $|\Upsilon^{|Q|\times |S|}$ and
  all ranks by $|Q| \times |S|$.
  It follows that the decision of whether there exists a (memoryless)
  combined weight-ranking for $B$ and $\cD$ and branching $\Upsilon$
  is in NP.
  \label{corollary:weight ranking memoryless limit}
\end{corollary}

%\begin{corollary}
%  The decision of whether there exists a (memoryless) combined
%  weight-ranking for $B$ and $\cD$ and branching $\Upsilon$ is in NP.
%  \label{corollary:buchi memoryless in NP}
%\end{corollary}

The proof of the corollary is given in Appendix. 

\subsection{Coverability with Memory}
\label{subsection:buchi memory}

We now turn to the more complicated case where a memory is required.
Notice that the example in Figure~\ref{figure:example buchi} requires
memory.
As mentioned, with the memory the notations become quite cumbersome.

Consider a transducer $\cD=\pair{\Psi,\Sigma,Q,\eta,q_0,L}$ and a 
DBW $B=\pair{\Upsilon\times\Sigma,S,\delta,s_0,F}$.
As before, we assume $q^\bot\notin Q$ and denote $Q^\bot=Q\cup
\{q^\bot\}$. 

A combined \emph{weight-ranking} for $B$ and $\cD$ with memory
$M$ is
$w:(Q\times S \times M) \cup (Q\times S \times M \times \Psi \times
\Upsilon \times M) \rightarrow \mathbb{N}$
and 
$d:Q^\bot \times S \times M \rightarrow (\mathbb{N} \cup \{\infty\})$
such that the following conditions hold.
\begin{compactitem}
\item
  For the weight distribution $w$ we have the following:
  \begin{compactitem}
  \item
    There is some $m_0\in M$ such that $w(q_0,s_0,m_0)=1$.
  \item
    For every $q\in Q$, $s\in S$, $m,m'\in M$, $\psi\in \Psi$, and
    $\upsilon\in\Upsilon$ if $w(q,s,m,\psi,\upsilon,m')>0$ then
    $\eta(q,\psi)$ and
    $\delta(s,(\upsilon,L(\eta(q,\psi))))$ are defined. 
  \item
    For every $q \in Q$, $s\in S$, and $m\in M$ we have 
    $|\Upsilon|\cdot w(q,s,m) \geq 
    \sum_{(\psi,\upsilon,m')}w(q,s,m,\psi,\upsilon,m')$.
  \item
    For every $q\in Q$, $s\in S$, $m\in M$, and $\upsilon \in
    \Upsilon$
    we have $\sum_{(\psi,m')}w(q,s,m,\psi,\upsilon,m') \leq w(q,s,m)$.
  \item
    For every $q\in Q$, $s\in S$, $m,m'\in M$, $\psi\in\Psi$, and $\upsilon
    \in \Upsilon$ we have $w(q,s,m,\psi,\upsilon,m') \geq
    w(\eta(q,\psi),\delta(s,(\upsilon,L(\eta(q,\psi)))),m')$.
  \end{compactitem}
\item
  For the ranking $d$ we have the following:
  \begin{compactitem}
  \item
    $d(q_0,s_0,m_0)\neq \infty$. 
  \item
    For every $s\notin B$ and for every $q\in Q$, $m\in M$, and
    $\upsilon \in \Upsilon$ such that $d(s,q,m)\neq \infty$: 
    \begin{compactitem}
    \item
      For every $\psi\in\Psi$ and $m'\in M'$
      such that  $w(q,s,m,\psi,\upsilon,m') >0$ we have 
      $d(q,s,m) >
      d(\eta(q,\psi),\delta(s,(\upsilon,L(\eta(q,\psi)))),m')$.
    \item
      If $\sum_{(\psi,m')}w(q,s,m,\psi,\upsilon,m')<w(q,s)$ then there
      is some $\sigma\in\Sigma$ and $m''\in M$ such that
      $d(q,s,m) > d(q^\bot,\delta(s,(\upsilon,\sigma)),m'')$.
    \end{compactitem}
  \item
    For every $s\in B$ and for every $q\in Q$, $m\in M$,
    and $\upsilon\in\Upsilon$ such that $d(s,q,m)\neq \infty$:
    \begin{compactitem}
    \item
      For every $\psi\in\Psi$ and $m'\in M'$ such that
      $w(q,s,m,\psi,\upsilon,m')>0$ we have
      $d(\eta(q,\psi),\delta(s,(\upsilon,L(\eta(q,\psi)))),m')\neq
      \infty$.
    \item
      If $\sum_{(\psi,m')}w(q,s,m,\psi,\upsilon,m')<w(q,s)$ then there
      is some $\sigma\in\Sigma$ such that 
      $d(q^\bot,\delta(s,(\upsilon,\sigma)),m'') \neq \infty$.
    \end{compactitem}
  \item
    If for some $s\in S$ and $m\in M$ we have $d(q^\bot,s,m)\neq \infty$ 
    then:
    \begin{compactitem}
    \item
      If $s\notin B$ then for every $\upsilon\in\Upsilon$ there is
      some $\sigma\in\Sigma$ and $m'\in M$ such that
      $d(q^\bot,s,m)>d(q^\bot,\delta(s,(\upsilon,\sigma)),m')$.
    \item
      If $s\in B$ then for every $\upsilon\in\Upsilon$ there is some
      $\sigma\in\Sigma$ and $m'\in M$ such that
      $d(q^\bot,\delta(s,(\upsilon,\sigma)),m')\neq \infty$. 
    \end{compactitem}
  \end{compactitem}
\end{compactitem}

This extends the previous definition with a memory value allowing to
make different choices in different locations in the tree.
This is required by the example in Figure~\ref{figure:example buchi}.

\begin{theorem}
  If for some memory domain $M$ there is a combined weight-ranking $w$
  and  $d$ for $B$ and $\cD$ with memory $M$ then
  the language of $\cD$ is coverable while realizing $B$ with 
  branching $\Upsilon$ 
\label{theorem:buchi coverability}
\end{theorem}

The proof, included in Appendix, adapts the ideas of the proof of
Theorem~\ref{theorem:buchi memoryless coverability} to include the
memory.


==> conc.tex <==
\section{Conclusions and Future Work}
\label{section:conclusions}

We consider the problem of realizability and synthesis with the
requirement to include a minimal set of behaviors.
We solve the problem in the case that there are no correctness
criteria and we have to ensure that the branching of the system is
sufficient to produce all required behaviors.
When  there are additional correctness criteria we show a
precondition for the existence of a solution.
We believe that these results are sufficient to merit
further study of the notion of coverability in the context of
realizability and synthesis.

The many future directions opened by this work include the following.
Is finite-memory sufficient for coverability
with realizability and is there an upper bound on the size of the required
memory?
Can these results be extended to more complicated specifications for
realizability?
How does one use coverability in practice to force more cooperative
systems?



==> figures/buchiaut1.tex <==
\newcommand\stack[2]{\begin{array}{c}{#1}\\{#2}\end{array}}
\aut{
\initial{1}{}{s_0}
\accept{2}{right of=1}{s_1^b}
\state{3}{below of=1}{s_1^a}
\state{4}{below of=2}{s_{2,3}}
\accept{5}{below of=3}{s_5}
\state{6}{below of=4}{s_4}

\fulledge{1}{3}{$(\mbox{*},c)$}{bend right}{left}
\fulledge{3}{1}{$(\beta,b)$}{bend right}{right,yshift=-3mm,xshift=-0.5mm}
\fulledge{2}{1}{$(\beta,b)$}{}{above}
\fulledge{3}{4}{$(\alpha,b)$}{}{below}
\fulledge{4}{2}{$(\mbox{*},c)$}{bend right}{right}
\fulledge{2}{4}{$(\alpha,b)$}{bend right}{left,yshift=3mm,xshift=0.5mm}
\fulledge{3}{5}{$(\mbox{*},a)$}{}{left}
\fulledge{4}{6}{$\stack{(\mbox{*},a)}{(\mbox{*},b)}$}{}{}
\fulledge{6}{5}{$(\mbox{*},b)$}{}{}
\fulledge{5}{5}{$\mbox{*}$}{loop left}{}
}


==> figures/ce1.tex <==
\aut{
\state{11}{}{\stackrel{s_3^5}{c}}
\state{12}{left of=11}{\stackrel{s_3^4}{c}}
\state{13}{left of=12}{\stackrel{s_3^3}{c}}
\state{14}{left of=13}{\stackrel{s_3^2}{c}}
\state{15}{left of=14}{\stackrel{s_3^1}{c}}

\state{22}{below of=12}{\stackrel{s_2^4}{b}}
\state{23}{left of=22}{\stackrel{s_2^3}{b}}
\state{24}{left of=23}{\stackrel{s_2^2}{b}}
\state{25}{left of=24}{\stackrel{s_2^1}{b}}

\state{32}{below of=22}{\stackrel{s_1^4}{a}}
\state{31}{right of=32}{\stackrel{s_1^5}{a}}
\state{33}{left of=32}{\stackrel{s_1^3}{a}}
\state{34}{left of=33}{\stackrel{s_1^2}{a}}
\initial{4}{left of=34}{\stackrel{s_1^1}{a}}

\fulledge{11}{11}{}{loop above}{}
\fulledge{11}{22}{}{}{}
\fulledge{31}{11}{}{bend right}{}
\fulledge{31}{22}{}{bend right=10}{}

\fulledge{12}{12}{}{loop above}{}
\fulledge{12}{31}{}{bend left=10}{}
\fulledge{12}{23}{}{}{}
\fulledge{22}{12}{}{}{}
\fulledge{22}{31}{}{bend right=10}{}
\fulledge{22}{23}{}{}{}
\fulledge{32}{31}{}{}{}
\fulledge{32}{12}{}{bend left}{}
\fulledge{32}{23}{}{bend right=10}{}

\fulledge{13}{13}{}{loop above}{}
\fulledge{13}{32}{}{bend left=10}{}
\fulledge{13}{24}{}{}{}
\fulledge{23}{13}{}{}{}
\fulledge{23}{32}{}{bend right=10}{}
\fulledge{23}{24}{}{}{}
\fulledge{33}{32}{}{}{}
\fulledge{33}{24}{}{bend right=10}{}
\fulledge{33}{13}{}{bend left}{}

\fulledge{14}{14}{}{loop above}{}
\fulledge{14}{33}{}{bend left=10}{}
\fulledge{14}{25}{}{}{}
\fulledge{24}{14}{}{}{}
\fulledge{24}{33}{}{bend right=10}{}
\fulledge{24}{25}{}{}{}
\fulledge{34}{33}{}{}{}
\fulledge{34}{14}{}{bend left}{}
\fulledge{34}{25}{}{bend right=10}{}

\fulledge{15}{15}{}{loop above}{}
\fulledge{15}{34}{}{bend left=10}{}
\fulledge{25}{15}{}{}{}
\fulledge{25}{34}{}{bend right=10}{}

\fulledge{4}{32}{}{bend right}{}
}


==> figures/ex1transducer.tex <==
\aut{
\initial{1}{}{b}
\state{2}{below of=1}{b}
\state{3}{below of=2}{b}
\state{5}{right of=2}{b}
\state{4}{above of=5}{a}
\state{6}{below of=5}{c}
\state{7}{right of=4}{a}
\state{8}{right of=5}{b}
\state{9}{right of=6}{c}
\edge{1}{2}
\edge{2}{3}
\edge{3}{4}
\edge{3}{5}
\edge{3}{6}
\edge{4}{7}
\edge{4}{8}
\edge{4}{9}
\edge{5}{7}
\edge{5}{8}
\edge{5}{9}
\edge{6}{7}
\edge{6}{8}
\edge{6}{9}

}

==> figures/ex1tree.tex <==
\aut{
\state{2121}{}{c}
\state{2112}{above of=2121,yshift=-8mm}{b}
\state{2111}{above of=2112,yshift=-8mm}{a}
\state{212}{left of=2121,xshift=5mm}{c}
\state{211}{left of=2111,xshift=5mm,yshift=-4mm}{c}
\state{1221}{above of=2111,yshift=-8mm}{c}
\state{1212}{above of=1221,yshift=-8mm}{b}
\state{1211}{above of=1212,yshift=-8mm}{a}
\state{122}{left of=1221,xshift=5mm}{b}
\state{121}{left of=1211,yshift=-4mm,xshift=5mm}{b}
\state{1121}{above of=1211,yshift=-8mm}{c}
\state{1112}{above of=1121,yshift=-8mm}{b}
\state{1111}{above of=1112,yshift=-8mm}{a}
\state{112}{left of=1121,xshift=5mm}{a}
\state{111}{left of=1111,yshift=-4mm,xshift=5mm}{a}
\state{21}{left of=211,yshift=-5mm,xshift=5mm}{b}
\state{12}{left of=121,yshift=-5mm,xshift=5mm}{b}
\state{11}{left of=111,yshift=-5mm,xshift=5mm}{b}
\state{2}{left of=21,xshift=5mm}{b}
\state{1}{left of=11,yshift=-11mm,xshift=5mm}{b}
\state{0}{left of=1,yshift=-17mm,xshift=5mm}{b}


\edge{0}{1}
\edge{0}{2}
\edge{1}{11}
\edge{1}{12}
\edge{2}{21}
\edge{11}{111}
\edge{11}{112}
\edge{12}{121}
\edge{12}{122}
\edge{21}{211}
\edge{21}{212}
\edge{111}{1111}
\edge{111}{1112}
\edge{112}{1121}
\edge{121}{1211}
\edge{121}{1212}
\edge{122}{1221}
\edge{211}{2111}
\edge{211}{2112}
\edge{212}{2121}
}
%\begin{center}
%\begin{tikzpicture}[scale=0.1]
%\tikzstyle{every node}+=[inner sep=0pt]
%\draw [black] (30.9,-37) circle (3);
%\draw (30.9,-37) node {$b$};
%\draw [black] (40.9,-22.9) circle (3);
%\draw (40.9,-22.9) node {$b$};
%\draw [black] (60.2,-28.3) circle (3);
%\draw (60.2,-28.3) node {$b$};
%\draw [black] (50.3,-33.7) circle (3);
%\draw (50.3,-33.7) node {$b$};
%\draw [black] (60.2,-9.2) circle (3);
%\draw (60.2,-9.2) node {$a$};
%\draw [black] (60.2,-47.9) circle (3);
%\draw (60.2,-47.9) node {$c$};
%\draw [black] (60.2,-18.6) circle (3);
%\draw (60.2,-18.6) node {$a$};
%\draw [black] (60.2,-38.2) circle (3);
%\draw (60.2,-38.2) node {$b$};
%\draw [black] (60.2,-57.9) circle (3);
%\draw (60.2,-57.9) node {$c$};
%\draw [black] (40.9,-52) circle (3);
%\draw (40.9,-52) node {$b$};
%\draw [black] (49.7,-52.8) circle (3);
%\draw (49.7,-52.8) node {$b$};
%\draw [black] (50.3,-14.1) circle (3);
%\draw (50.3,-14.1) node {$b$};
%\draw [black] (70.5,-5.5) circle (3);
%\draw (70.5,-5.5) node {$a$};
%\draw [black] (70.5,-12.1) circle (3);
%\draw (70.5,-12.1) node {$b$};
%\draw [black] (70.5,-18.6) circle (3);
%\draw (70.5,-18.6) node {$c$};
%\draw [black] (70.5,-25.2) circle (3);
%\draw (70.5,-25.2) node {$a$};
%\draw [black] (70.5,-31.8) circle (3);
%\draw (70.5,-31.8) node {$b$};
%\draw [black] (70.5,-38.2) circle (3);
%\draw (70.5,-38.2) node {$c$};
%\draw [black] (70.5,-44.6) circle (3);
%\draw (70.5,-44.6) node {$a$};
%\draw [black] (70.5,-51.2) circle (3);
%\draw (70.5,-51.2) node {$b$};
%\draw [black] (70.5,-57.9) circle (3);
%\draw (70.5,-57.9) node {$c$};
%\draw [black] (32.64,-34.55) -- (39.16,-25.35);
%\fill [black] (39.16,-25.35) -- (38.29,-25.71) -- (39.11,-26.29);
%\draw [black] (42.87,-25.16) -- (48.33,-31.44);
%\fill [black] (48.33,-31.44) -- (48.18,-30.51) -- (47.43,-31.16);
%\draw [black] (32.56,-39.5) -- (39.24,-49.5);
%\fill [black] (39.24,-49.5) -- (39.21,-48.56) -- (38.38,-49.12);
%\draw [black] (43.89,-52.27) -- (46.71,-52.53);
%\fill [black] (46.71,-52.53) -- (45.96,-51.96) -- (45.87,-52.95);
%\draw [black] (43.09,-20.85) -- (48.11,-16.15);
%\fill [black] (48.11,-16.15) -- (47.18,-16.33) -- (47.87,-17.06);
%\draw [black] (52.99,-12.77) -- (57.51,-10.53);
%\fill [black] (57.51,-10.53) -- (56.57,-10.44) -- (57.02,-11.33);
%\draw [black] (53.03,-15.34) -- (57.47,-17.36);
%\fill [black] (57.47,-17.36) -- (56.95,-16.57) -- (56.53,-17.48);
%\draw [black] (52.93,-32.26) -- (57.57,-29.74);
%\fill [black] (57.57,-29.74) -- (56.62,-29.68) -- (57.1,-30.56);
%\draw [black] (53.03,-34.94) -- (57.47,-36.96);
%\fill [black] (57.47,-36.96) -- (56.95,-36.17) -- (56.53,-37.08);
%\draw [black] (52.42,-51.53) -- (57.48,-49.17);
%\fill [black] (57.48,-49.17) -- (56.55,-49.05) -- (56.97,-49.96);
%\draw [black] (52.5,-54.2) -- (57.5,-56.6);
%\fill [black] (57.5,-56.6) -- (56.99,-55.8) -- (56.56,-56.7);
%\draw [black] (63.2,-57.9) -- (67.5,-57.9);
%\fill [black] (67.5,-57.9) -- (66.7,-57.4) -- (66.7,-58.4);
%\draw [black] (63.06,-48.82) -- (67.64,-50.28);
%\fill [black] (67.64,-50.28) -- (67.03,-49.56) -- (66.73,-50.52);
%\draw [black] (63.06,-46.98) -- (67.64,-45.52);
%\fill [black] (67.64,-45.52) -- (66.73,-45.28) -- (67.03,-46.24);
%\draw [black] (63.2,-38.2) -- (67.5,-38.2);
%\fill [black] (67.5,-38.2) -- (66.7,-37.7) -- (66.7,-38.7);
%\draw [black] (63.04,-29.27) -- (67.66,-30.83);
%\fill [black] (67.66,-30.83) -- (67.06,-30.1) -- (66.74,-31.05);
%\draw [black] (63.07,-27.44) -- (67.63,-26.06);
%\fill [black] (67.63,-26.06) -- (66.72,-25.82) -- (67.01,-26.77);
%\draw [black] (63.2,-18.6) -- (67.5,-18.6);
%\fill [black] (67.5,-18.6) -- (66.7,-18.1) -- (66.7,-19.1);
%\draw [black] (63.09,-10.01) -- (67.61,-11.29);
%\fill [black] (67.61,-11.29) -- (66.98,-10.59) -- (66.71,-11.55);
%\draw [black] (63.02,-8.19) -- (67.68,-6.51);
%\fill [black] (67.68,-6.51) -- (66.75,-6.31) -- (67.09,-7.26);
%\end{tikzpicture}
%\end{center}

==> figures/ex2buchitree.tex <==
\aut{
%\state{21}{}{c}
\state{12}{}{b}
\state{121}{right of=12,xshift=-5mm}{b}
\state{11}{above of=12,yshift=-8mm}{a}
\state{111}{right of=11,xshift=-5mm}{b}
\state{2}{below of=12,yshift=5mm,xshift=-10mm}{b}
\state{1}{left of=11,xshift=5mm,yshift=-4mm}{b}
\state{0}{left of=1,yshift=-6mm,xshift=5mm}{c}
\state{21}{below of=12,yshift=8mm}{c}
\state{22}{below of=21,yshift=8mm}{c}
%\state{211}{below of=121}{b}
%\state{221}{below of=211}{b}
\fulledge{1}{11}{$\alpha$}{}{xshift=4pt,yshift=-5pt}
\fulledge{1}{12}{$\beta$}{}{xshift=-6pt,yshift=-5pt}
\fulledge{0}{1}{$\alpha$}{}{xshift=4pt,yshift=-5pt}
\fulledge{0}{2}{$\beta$}{}{below,xshift=-4pt,yshift=5pt}
\fulledge{12}{121}{$\alpha$}{}{yshift=-3pt}
\fulledge{11}{111}{$\alpha$}{}{yshift=-3pt}
\fulledge{2}{21}{$\alpha$}{}{xshift=5pt,yshift=-4pt}
\fulledge{2}{22}{$\beta$}{}{below,xshift=-4pt,yshift=4pt}
\fulledge{21}{1}{$\alpha$}{dashed}{xshift=5pt,yshift=5pt}
\fulledge{22}{2}{$\alpha$}{dashed,bend left=60}{xshift=4pt,yshift=5pt}
}
%
%\begin{center}
%\begin{tikzpicture}[scale=0.1]
%\tikzstyle{every node}+=[inner sep=0pt]
%\draw [black] (35.2,-29.9) circle (3);
%\draw (35.2,-29.9) node {$b$};
%\draw [black] (46.8,-29.9) circle (3);
%\draw (46.8,-29.9) node {$c$};
%\draw [black] (46.9,-6.9) circle (3);
%\draw (46.9,-6.9) node {$a$};
%\draw [black] (59.2,-6.9) circle (3);
%\draw (59.2,-6.9) node {$b$};
%\draw [black] (46.8,-19.2) circle (3);
%\draw (46.8,-19.2) node {$b$};
%\draw [black] (59.2,-19.2) circle (3);
%\draw (59.2,-19.2) node {$b$};
%\draw [black] (35.2,-12.4) circle (3);
%\draw (35.2,-12.4) node {$b$};
%\draw [black] (24.1,-20.6) circle (3);
%\draw (24.1,-20.6) node {$c$};
%\draw [black] (26.51,-18.82) -- (32.79,-14.18);
%\fill [black] (32.79,-14.18) -- (31.85,-14.26) -- (32.44,-15.06);
%\draw [black] (26.4,-22.53) -- (32.9,-27.97);
%\fill [black] (32.9,-27.97) -- (32.61,-27.08) -- (31.97,-27.84);
%\draw [black] (38.2,-29.9) -- (43.8,-29.9);
%\fill [black] (43.8,-29.9) -- (43,-29.4) -- (43,-30.4);
%\draw [black] (37.79,-13.92) -- (44.21,-17.68);
%\fill [black] (44.21,-17.68) -- (43.77,-16.85) -- (43.27,-17.71);
%\draw [black] (37.91,-11.12) -- (44.19,-8.18);
%\fill [black] (44.19,-8.18) -- (43.25,-8.06) -- (43.67,-8.97);
%\draw [black] (50.2,-6.9) -- (56.2,-6.9);
%\fill [black] (56.2,-6.9) -- (55.4,-6.4) -- (55.4,-7.4);
%\draw [black] (49.8,-19.2) -- (56.2,-19.2);
%\fill [black] (56.2,-19.2) -- (55.4,-18.7) -- (55.4,-19.7);
%\draw [black] (44.754,-32.085) arc (-49.92039:-174.63662:12.644);
%\fill [black] (24.03,-23.59) -- (23.6,-24.44) -- (24.6,-24.34);
%\end{tikzpicture}
%\end{center}


==> figures/ex2transducer.tex <==
\newcommand\stack[2]{\begin{array}{c}{#1}\\{#2}\end{array}}
\aut{
\initial{1}{}{\begin{array}{c}q_0\\c\end{array}}
\state{2}{right of=1}{\stack{q_1}{b}}
\state{3}{right of=2,yshift=5mm}{\stack{q_2}{a}}
\state{4}{right of=2,yshift=-5mm}{\stack{q_3}{b}}
\state{5}{right of=3,yshift=-5mm}{\stack{q_4}{b}}
\fulledge{1}{2}{}{bend right}{}
\fulledge{2}{1}{}{bend right}{}
\edge{2}{3}
\edge{2}{4}
\edge{3}{5}
\edge{4}{5}
}
%\begin{center}
%\begin{tikzpicture}[scale=0.1]
%\tikzstyle{every node}+=[inner sep=0pt]
%\draw [black] (18.9,-12.6) circle (3);
%\draw (18.9,-12.6) node {$c$};
%\draw [black] (33.4,-12.8) circle (3);
%\draw (33.4,-12.8) node {$b$};
%\draw [black] (46.9,-6.9) circle (3);
%\draw (46.9,-6.9) node {$a$};
%\draw [black] (58.4,-12.8) circle (3);
%\draw (58.4,-12.8) node {$b$};
%\draw [black] (46.8,-19.2) circle (3);
%\draw (46.8,-19.2) node {$b$};
%\draw [black] (12.8,-12.6) -- (15.9,-12.6);
%\fill [black] (15.9,-12.6) -- (15.1,-12.1) -- (15.1,-13.1);
%\draw [black] (31.386,-15.003) arc (-52.53497:-129.0455:8.507);
%\fill [black] (31.39,-15) -- (30.45,-15.09) -- (31.06,-15.89);
%\draw [black] (36.15,-11.6) -- (44.15,-8.1);
%\fill [black] (44.15,-8.1) -- (43.22,-7.96) -- (43.62,-8.88);
%\draw [black] (36.11,-14.09) -- (44.09,-17.91);
%\fill [black] (44.09,-17.91) -- (43.59,-17.11) -- (43.16,-18.01);
%\draw [black] (20.506,-10.088) arc (136.31725:42.10228:7.752);
%\fill [black] (20.51,-10.09) -- (21.42,-9.86) -- (20.7,-9.16);
%\draw [black] (49.57,-8.27) -- (55.73,-11.43);
%\fill [black] (55.73,-11.43) -- (55.25,-10.62) -- (54.79,-11.51);
%\draw [black] (49.43,-17.75) -- (55.77,-14.25);
%\fill [black] (55.77,-14.25) -- (54.83,-14.2) -- (55.31,-15.07);
%\end{tikzpicture}
%\end{center}


==> figures/ex2tree.tex <==
\aut{
%\state{21}{}{c}
\state{12}{}{b}
\state{121}{right of=12,xshift=-5mm}{b}
\state{11}{above of=12,yshift=-8mm}{a}
\state{111}{right of=11,xshift=-5mm}{b}
\state{2}{below of=12,yshift=8mm,xshift=-10mm}{b}
\state{1}{left of=11,xshift=5mm,yshift=-4mm}{b}
\state{0}{left of=1,yshift=-5mm,xshift=5mm}{c}
\edge{1}{11}
\edge{1}{12}
\fulledge{2}{0}{}{dashed,bend left=60}{}
\edge{0}{1}
\edge{0}{2}
\edge{12}{121}
\edge{11}{111}
}
%
%\begin{center}
%\begin{tikzpicture}[scale=0.1]
%\tikzstyle{every node}+=[inner sep=0pt]
%\draw [black] (35.2,-29.9) circle (3);
%\draw (35.2,-29.9) node {$b$};
%\draw [black] (46.8,-29.9) circle (3);
%\draw (46.8,-29.9) node {$c$};
%\draw [black] (46.9,-6.9) circle (3);
%\draw (46.9,-6.9) node {$a$};
%\draw [black] (59.2,-6.9) circle (3);
%\draw (59.2,-6.9) node {$b$};
%\draw [black] (46.8,-19.2) circle (3);
%\draw (46.8,-19.2) node {$b$};
%\draw [black] (59.2,-19.2) circle (3);
%\draw (59.2,-19.2) node {$b$};
%\draw [black] (35.2,-12.4) circle (3);
%\draw (35.2,-12.4) node {$b$};
%\draw [black] (24.1,-20.6) circle (3);
%\draw (24.1,-20.6) node {$c$};
%\draw [black] (26.51,-18.82) -- (32.79,-14.18);
%\fill [black] (32.79,-14.18) -- (31.85,-14.26) -- (32.44,-15.06);
%\draw [black] (26.4,-22.53) -- (32.9,-27.97);
%\fill [black] (32.9,-27.97) -- (32.61,-27.08) -- (31.97,-27.84);
%\draw [black] (38.2,-29.9) -- (43.8,-29.9);
%\fill [black] (43.8,-29.9) -- (43,-29.4) -- (43,-30.4);
%\draw [black] (37.79,-13.92) -- (44.21,-17.68);
%\fill [black] (44.21,-17.68) -- (43.77,-16.85) -- (43.27,-17.71);
%\draw [black] (37.91,-11.12) -- (44.19,-8.18);
%\fill [black] (44.19,-8.18) -- (43.25,-8.06) -- (43.67,-8.97);
%\draw [black] (50.2,-6.9) -- (56.2,-6.9);
%\fill [black] (56.2,-6.9) -- (55.4,-6.4) -- (55.4,-7.4);
%\draw [black] (49.8,-19.2) -- (56.2,-19.2);
%\fill [black] (56.2,-19.2) -- (55.4,-18.7) -- (55.4,-19.7);
%\draw [black] (44.754,-32.085) arc (-49.92039:-174.63662:12.644);
%\fill [black] (24.03,-23.59) -- (23.6,-24.44) -- (24.6,-24.34);
%\end{tikzpicture}
%\end{center}


==> figures/ex3transducer.tex <==
\aut{
\initial{1}{}{\stackrel{\scriptsize \alpha}{c}}
\labeln{1}{text=red,left of=1,xshift=12mm,yshift=-3.5mm}{1}
\state{2}{above of=1}{\stackrel{\scriptsize \beta}{c}}
\labeln{2}{text=red,left of=2,xshift=12mm,yshift=3.5mm}{2}
\state{3}{right of=1}{\stackrel{\scriptsize \gamma}{a}}
\labeln{3}{text=red,left of=3,xshift=19mm}{2}
\state{4}{above of=3}{\stackrel{\scriptsize \delta}{b}}
\labeln{4}{text=red,left of=4,xshift=12mm,yshift=3mm}{1}
\state{5}{right of=3}{\stackrel{\scriptsize \epsilon}{a}}
\labeln{5}{text=red,left of=5,xshift=19mm,yshift=-3.5mm}{1}
\state{6}{above of=5}{\stackrel{\scriptsize \varphi}{b}}
\labeln{6}{text=red,left of=6,xshift=19mm,yshift=3.5mm}{2}
\fulledge{2}{1}{1}{}{text=blue,xshift=-4.5mm,yshift=3mm}
\fulledge{2}{4}{1}{}{text=blue,yshift=-4.5mm,xshift=-3mm}
\fulledge{2}{3}{2}{}{text=blue,xshift=-8.5mm}
\fulledge{1}{3}{2}{bend left}{text=blue,yshift=-2mm,xshift=-4mm}
\fulledge{3}{1}{1}{bend left}{text=blue,xshift=4mm,yshift=2mm}
\fulledge{3}{3}{2}{loop below}{text=blue,xshift=2.5mm,yshift=6mm}
\fulledge{3}{4}{1}{}{text=blue,xshift=4.5mm,yshift=-3mm}
\fulledge{4}{6}{2}{}{text=blue,xshift=-3.5mm,yshift=-5mm}
\fulledge{5}{6}{2}{bend left}{text=blue,xshift=2.5mm,yshift=-4mm}
\fulledge{6}{2}{2}{bend right}{text=blue,xshift=12mm,yshift=2mm}
\fulledge{6}{5}{1}{bend left}{text=blue,xshift=-2.5mm,yshift=4mm}
}


==> figures/ex3tree.tex <==
\aut{
\state{0}{}{c}
\state{1}{right of=0,yshift=7mm}{a}
\state{2}{right of=0,yshift=-7mm}{a}
\state{21}{right of=2}{b}
\state{211}{right of=21,yshift=7mm}{b}
\state{212}{right of=21,yshift=-7mm}{b}
\state{2111}{right of=211,yshift=7mm}{c}
\state{2112}{right of=211,yshift=-7mm}{c}
\state{2121}{right of=212,yshift=-7mm}{a}
\edge{0}{1}
\edge{0}{2}
\edge{2}{21}
\edge{21}{211}
\edge{21}{212}
\fulledge{1}{0}{}{dashed,bend right}{}
\fulledge{1}{1}{}{loop above,dashed}{}
\fulledge{2}{2}{}{loop above,dashed}{}
\edge{211}{2111}
\edge{211}{2112}
\edge{212}{2121}
\fulledge{2111}{0}{}{dashed}{}
\fulledge{2111}{1}{}{dashed}{}
\fulledge{2112}{2}{}{dashed,bend left=15}{}
\fulledge{2112}{21}{}{dashed}{}
\fulledge{2121}{212}{}{dashed,bend left}{}
\fulledge{2121}{211}{}{dashed}{}
}


==> figures/exbuchinot.tex <==
\aut{
\initial{1}{}{c}
\state{2}{right of=1,xshift=-2mm}{b}
\state{3}{right of=2,yshift=5mm,xshift=-2mm}{a}
\state{4}{right of=2,yshift=-5mm,xshift=-2mm}{b}
\state{5}{right of=3,yshift=-5mm,xshift=-2mm}{b}
\state{6}{above of=5,yshift=-5mm,xshift=-2mm}{a}
\state{7}{below of=5,yshift=5mm,xshift=-2mm}{c}
\fulledge{1}{2}{}{bend right}{}
\fulledge{2}{1}{}{bend right}{}
\edge{2}{3}
\edge{2}{4}
\edge{3}{5}
\edge{4}{5}
\edge{3}{6}
\edge{3}{7}
\edge{4}{7}
}
%\begin{center}
%\begin{tikzpicture}[scale=0.1]
%\tikzstyle{every node}+=[inner sep=0pt]
%\draw [black] (18.9,-12.6) circle (3);
%\draw (18.9,-12.6) node {$c$};
%\draw [black] (33.4,-12.8) circle (3);
%\draw (33.4,-12.8) node {$b$};
%\draw [black] (46.9,-6.9) circle (3);
%\draw (46.9,-6.9) node {$a$};
%\draw [black] (58.4,-12.8) circle (3);
%\draw (58.4,-12.8) node {$b$};
%\draw [black] (46.8,-19.2) circle (3);
%\draw (46.8,-19.2) node {$b$};
%\draw [black] (12.8,-12.6) -- (15.9,-12.6);
%\fill [black] (15.9,-12.6) -- (15.1,-12.1) -- (15.1,-13.1);
%\draw [black] (31.386,-15.003) arc (-52.53497:-129.0455:8.507);
%\fill [black] (31.39,-15) -- (30.45,-15.09) -- (31.06,-15.89);
%\draw [black] (36.15,-11.6) -- (44.15,-8.1);
%\fill [black] (44.15,-8.1) -- (43.22,-7.96) -- (43.62,-8.88);
%\draw [black] (36.11,-14.09) -- (44.09,-17.91);
%\fill [black] (44.09,-17.91) -- (43.59,-17.11) -- (43.16,-18.01);
%\draw [black] (20.506,-10.088) arc (136.31725:42.10228:7.752);
%\fill [black] (20.51,-10.09) -- (21.42,-9.86) -- (20.7,-9.16);
%\draw [black] (49.57,-8.27) -- (55.73,-11.43);
%\fill [black] (55.73,-11.43) -- (55.25,-10.62) -- (54.79,-11.51);
%\draw [black] (49.43,-17.75) -- (55.77,-14.25);
%\fill [black] (55.77,-14.25) -- (54.83,-14.2) -- (55.31,-15.07);
%\end{tikzpicture}
%\end{center}


==> finite.tex <==
\section{Simple Covering}
\label{section:simple}

Solutions to realizability problems include two-player games or tree 
automata.
The problem we are interested in here is dual.
Instead (and later in addition to) of requiring that all interactions
between the system and its environment produce computations that
satisfy the specification, here we require that a minimal set of computations 
(produced by a finite transducer) are generated by the interactions.

Consider an alphabet $\Sigma$, and two sets of directions $\Upsilon$ and $\Psi$. 
Consider a transducer $\cD=\pair{\Psi,\Sigma,Q,\eta,q_0,L}$.
We say that $T=\pair{\Upsilon^*,\tau}$ covers $L(\cD)$ if
$L(T) \supseteq L(\cD)$.
We note that the set $\Psi$ helps to distinguish between transitions
of $\cD$ but does not appear on $T$. 

\begin{definition}{\rm Covering.}
  The language of a transducer $\cD$ is coverable with branching $\Upsilon$ 
  if there is a labeled $\Upsilon$-tree $T$ that covers $L(\cD)$.
\end{definition}

Obviously, the question makes sense only in the case that $|\Upsilon|
< |\Sigma|$ and $|\Upsilon|<|\Psi|$.
If $|\Upsilon|\geq |\Sigma|$ then it is trivial to label an 
$\Upsilon$-tree by $\Sigma^*$.
If  $|\Upsilon|\geq |\Psi|$ we can use the regular tree
induced by $\cD$ as a subset of $\Upsilon^*$.

\begin{figure}[bt]
\begin{minipage}{0.5\textwidth}
\input{figures/ex1transducer.tex}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\input{figures/ex1tree.tex}
\end{minipage}
%\includegraphics[width=\textwidth]{03_example1.jpg}
\vspace*{-3mm}
\caption{\label{figure:example 1}A transducer whose language is coverable and a 
tree witnessing it.}
\vspace*{-6mm}
\end{figure}

Consider for example the transducer in Figure~\ref{figure:example 1}. 
The language of the transducer is finite and 
includes only 9 words. 
The alphabet is $\{a,b,c\}$ and the language is $b^3\{a,b,c\}^2$, that is, all words 
of length 5 that start with three $b$s.
We include an example of a tree of branching degree $2$ (i.e.,
$|\Upsilon|=2$) that covers this language. 
Clearly, in the case of branching degree $3$ or more (i.e., $|\Upsilon|\geq 3$) 
the language is trivially coverable as $|\Sigma|=3$.

\begin{figure}[bt]
\begin{minipage}{0.5\textwidth}
\input{figures/ex2transducer.tex}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\input{figures/ex2tree.tex}
\end{minipage}
  \vspace*{-8mm}
%\includegraphics[width=\textwidth]{04_example2.jpg}
\caption{\label{figure:example 2}A coverable transducer with infinite
  language and a tree witnessing it.} 
\vspace*{-6mm}
\end{figure}

We proceed with a slightly more complicated example. 
Consider the transducer in Figure~\ref{figure:example 2}.
As before, the alphabet is $\{a,b,c\}$ and for now we can ignore the
state names. 
This time, the language is infinite: $(cb)^*\{a,b\}b$. That is, start
with a finite number of $cb$s and follow with an $a$ or a $b$ and a
final $b$. 
Again, when $|\Upsilon|=2$ there is a tree covering the language and
we include such an example. 
As before, if $|\Upsilon|\geq 3$ then coverability is trivial.

\begin{figure}[bt]
%\includegraphics[width=\textwidth]{05_counterexample1.jpg}
  \input{figures/ce1.tex}
  \vspace*{-8mm}
\caption{\label{figure:counter example 1}A transducer whose language
  is not coverable with branching degree $2$.} 
\vspace*{-6mm}
\end{figure}

Finally, consider the example in Figure~\ref{figure:counter example 1}. 
The alphabet is $\{a,b,c\}$ as before.
For a letter $\sigma\in\Sigma$ we denote $\#_\sigma(w)$ the number of
occurrences of $\sigma$ in $w$. 
A word $u$ is a prefix of $w$ if $w=u\cdot v$ for some $v$, denoted by
$u\leq w$. 
Then, the language of the transducer is 
$\{w ~|~ \forall u\leq w. |\#_a(u)-\#_b(u)| \leq 2\mbox{ and } w_0=a\}$.
Indeed, in the states in the middle column ($s_1^3$, $s_2^3$, and
$s_3^3$) and the initial state the number of $a$s and $b$s seen so far
is equal.
Then, an increase in the number of $a$s moves to the right.
From the right-most column (states with superscript $5$, where two
$a$s have been seen more than $b$s, it is impossible to read further
$a$s until another $b$ is read.
This language is not coverable with branching degree $2$. 
We are going to develop the tools that will enable us to prove this.
But, intuitively, in a hypothetical tree covering this language there
should be two nodes below the root of the tree that correspond to
state $s_1^4$.
Indeed, otherwise, it would be impossible to cover the three
possible continuations of $aa$, namely  
$aaa$, $aab$, and $aac$.
For exactly the same reason, two nodes in level $2$ of the tree must
correspond to state $s_3^4$ and two to state $s_2^3$ (the
$c$-successor and the $b$-successor).
As there are only four nodes in level two of the tree this leaves no
free nodes to cover the runs leading to state $s_1^5$, the
$a$-successor of $s_1^4$.
We make this argument formal in what follows.

Consider a transducer $\cD=\pair{\Psi,\Sigma,Q,\eta,q_0,L}$. 
We denote $(q,\psi,q')\in \eta$ for $q' = \eta(q,\psi)$. 
A \emph{weight distribution} for $\cD$ and branching $\Upsilon$
is a function $w:Q\cup (Q \times \Psi \times Q) \rightarrow \mathbb{N}$
such that the following conditions hold. 
\begin{compactitem}
\item
$w(q_0) =1$
\item
For every $q\in Q$ we have $|\Upsilon|\cdot w(q) \geq
\sum_{(q,\psi,q')\in \eta} w(q,\psi,q')$.

That is, the weight of $q$ can cover the weights of all
outgoing transitions. 
\item
For every $(q,\psi,q')\in \eta$ we have $w(q,\psi,q')\geq w(q')$ and
$w(q,\psi,q')>0$.

That is, the weight of a transition can cover the target
of that transition. 
\end{compactitem}

Intuitively, with $w(q)$ nodes in the tree we can cover the language of
$\cD_q$, namely $\cD$ with $q$ as its initial state. 
The language of $\cD_q$ is covered by allocating $w(q,\psi,q')$
of the children of the $w(q)$ nodes to successor $q'$.
As $|\Upsilon|\cdot w(q)\geq \sum_{(q,\psi,q')\in \eta}w(q,\psi,q')$ we
have enough children for all successors of $q$.
As $w(q,\psi,q') \geq w(q')$ the children allocated for $q'$ are
sufficient to cover the language of $\cD_{q'}$. 


\begin{figure}[bt]
%  \includegraphics[width=\textwidth]{06_example3.jpg}
\begin{minipage}{0.4\textwidth}
\input{figures/ex3transducer.tex}
\end{minipage}
\begin{minipage}{0.6\textwidth}
\input{figures/ex3tree.tex}
\end{minipage}
\vspace*{-6mm}
\caption{\label{figure:example 3}
A coverable transducer with its weight distribution (state weights
in red and transition weights in blue) and the corresponding witness tree.}
\vspace*{-6mm}
\end{figure}

Consider the transducer in Figure~\ref{figure:example 3}. 
Its alphabet is $\Sigma=\{a,b,c\}$ and we consider $|\Upsilon|=2$.
The numbers written on states (red) and transitions (blue) constitute
a weight distribution. 
Indeed, for the initial state, we have $w(\alpha)=1$ and
$2w(\alpha)\geq w(\alpha,.,\gamma)$. 
Also, $w(\alpha) \leq w(\beta,.,\alpha)$ and $w(\alpha)\leq
w(\gamma,.,\alpha)$. 
For state $\gamma$, we have $w(\gamma)=2$, which is also the weight of
the three incoming transitions $(\alpha,.,\gamma)$,
$(\beta,.,\gamma)$, and $(\gamma,.,\gamma)$.
Also $2w(\gamma) \geq w(\gamma,.,\alpha) + w(\gamma,.,\gamma) +
w(\gamma,.,\delta)$.
The conditions for the other states and transitions can be verified as
well.

We also go back to the transducer in
Figure~\ref{figure:counter example 1} and show that it is not
coverable with branching degree $2$. 
As $w(s_1^1)=1$ the maximal weight for the transition to $s_1^4$ is $2$
implying that $w(s_1^4)\geq 2$. 
Suppose that $w(s_1^4)=2$. 
Then $w(s_1^4,.,s_3^4)$ must be at least $2$ as well as the two states
have the same language after the initial symbol.
It follows that both $w(s_1^4,.,s_1^5)$ and $w(s_1^4,.,s_2^3)$ are 1.
As $w(s_1^4,.,s_2^3)=1$ it must be that $w(s_2^3)\leq 1$, which
contradicts $2w(s_2^3)\geq 3$.
Suppose that $w(s_1^4)=n>2$. 
As before $w(s_1^4,.,s_3^4)\geq n$ implying that $w(s_1^4,.,s_2^3)<n$
and $w(s_2^3)<n$. 
Applying the same logic to $w(s_2^3,.,s_3^3)$, we conclude that
$w(s_2^3,.,s_1^4)<n$. 
This contradicts $w(s_2^3,.,s_1^4)\geq w(s_1^4)$. 
This shows that the language of this transducer cannot be covered by a
tree of branching degree 2.
In fact, for every $n$, the language $a^nL(\cD)$ cannot be
covered by a tree of branching degree 2.


We show that the language of $\cD$ is coverable if and only if
there exists a weight distribution for $\cD$.
Intuitively, the weight tells us how many nodes in the tree should
correspond to a state of the transducer (following a certain
transition).

\begin{theorem}
The language of $\cD$ is coverable by an $\Upsilon$-tree if and
only if there is a weight distribution $w$ for $\cD$ and
branching $\Upsilon$.
\label{theorem:finite coverability}
\end{theorem}

\begin{proof}
\begin{compactitem}
\item[$\Leftarrow$]
We construct an $\Upsilon$-tree covering $\cD$ from a weight distribution.

Consider the tree $\Upsilon^*$.
Based on the weight distribution $w$, we construct a $Q^+$-labeled  
$\Upsilon$-tree $T=\pair{\Upsilon^*,\pi}$ by induction, where the
labeling may be partial. 
The labeling maintains the following:
\begin{itemize}
\item
  for every $x\in \Upsilon^*$ we have $|x|+1=|\pi(x)|$.
\item
  for every run $r\in Q^+$ of $\cD$ ending in state
  $q$, we maintain the invariant that there are at least $w(q)$ nodes
  $\{x_1,\ldots, x_{w(q)}\}$ in $\Upsilon^*$ such that for every $i$
  we have $\pi(x_i)=r$.
\item
  for every $x\upsilon\in \Upsilon^+$ if $\pi(x\upsilon)=rqq'$
  then $\pi(x)=r\cdot q$ for some $q'$ such that $(q,\psi,q')\in
  \eta$.
  
  That is, the nodes in the tree are labeled by runs of
  $\cD$ and children of a node are labeled by runs that extend the
  run labeling their parent.
\end{itemize}

We set $\pi(\varepsilon)=q_0$. 
Clearly, $|\varepsilon|+1=|q_0|$.
By definition of weight distribution $w(q_0)=1$ and hence one node
$\varepsilon$ labeled by the run $q_0$ is sufficient. 

Consider a run $r$ ending in state $q$ and let $X=\{x_1,\ldots,
x_{w(q)}\}\subset \Upsilon^*$ such  
that for every $i$ we have $\pi(x_i)=r$.
By definition of the weight distribution we have 
$|\Upsilon|\cdot w(q) \geq \sum_{(q,\psi,q')\in \eta} w(q,\psi,q')$
and for every  
$(q,\psi,q')\in \eta$ we have $w(q,\psi,q')\geq w(q')$.
Let $Y$ denote the set of nodes 
$\{x\cdot \upsilon ~|~ x\in X \mbox{ and } \upsilon \in \Upsilon\}$.
It follows that $|Y|=|\Upsilon|\times w(q)$.
Hence, we can partition $Y$ such that for every $(q,\psi,q')\in \eta$
there is a set  
$Y_{(q,\psi,q')}$ of size $w(q,\psi,q')$ such that for every two
$(q,\psi,q')$ and  
$(q,\psi',q'')$ such that $\psi\neq \psi'$ we have 
$Y_{(q,\psi,q')}\cap Y_{(q,\psi',q'')}=\emptyset$.
It follows that it is safe to label the nodes $x\upsilon\in
Y_{(q,\psi,q')}$ by the run $\pi(x)\cdot q'$.
That is, for $x\upsilon \in Y_{(q,\psi,q')}$ we set
$\pi(x\upsilon)=\pi(x)\cdot q'$. 

As $w(q,\psi,q')\geq w(q')$ there are at least $w(q')$ nodes labeled
by $r\cdot q'$.  
As $|x|+1=|r|$ then $|x\upsilon|+1=|rq'|$.
Finally, $\pi(x\upsilon)$ extends $\pi(x)$ by $q'$. 

This completes the construction of $\pi$ by induction.
We now use $\pi$ to show a labeling $\tau$ for $\Upsilon^*$ that
covers the language of $\cD$.
By the invariant for labeling, for every run $r$ of $\cD$ there
is (at least) a  
node $x\in \Upsilon$ such that $\pi(x)=r$.
We set $\tau(x)=L(q)$, where $q$ is the last state of
$\pi(x)$.
As required, $L(\cD)\subseteq L(T)$. 
\item[$\Rightarrow$]
Consider a tree $T=\pair{\Upsilon^*,\tau}$ such that $L(\cD)
\subseteq L(T)$. 
As $\cD$ is deterministic, we can create a mapping
$\pi:\Upsilon^*\rightarrow Q^+$ mapping 
every node $x$ of $\Upsilon^*$ to the run of $\cD$ corresponding
to $\vec{\tau}(x)$. 

Let $R$ denote the set of runs of $\cD$.
For every state $q\in Q$, let $w(q)$ denote 
$\displaystyle\min_{rq\in R} |\{x\in \Upsilon^* ~|~ \pi(x)=rq\}$. 
That is, of all the runs ending in $q$, all of them appearing in the
tree $T$, consider  
the one that has the minimal number of copies in $T$.
For a state $q$, let $X_q=\{x_1,\ldots, x_{w(q)}\}$ denote the set of
nodes of $\Upsilon^*$  
such that there is a run $rq$ of $\cD$ and for every $i$ we have
$\pi(x_i)=rq$, where $rq$  
gives rise to the minimal such set.
Consider a transition $(q,\psi,q')$ of $\cD$.
Clearly, all the runs $rqq'$ have to appear in $T$.
Let
$$
Y_{(q,\psi,q')} = \{x\cdot \upsilon ~|~ x\in X_q,~
\upsilon\in\Upsilon, \mbox{ and } \pi(x\cdot \upsilon)=rqq'\}.
$$
Clearly, as $X_q$ includes all nodes such that $r(x)=rq$ we have
$Y_{(q,\psi,q')}$ includes all nodes such that $r(x)=rqq'$. 
We set $w(q,\psi,q')=|Y_{(q,\psi,q')}|$.

By definition $q_0$ must label the root of the tree $\varepsilon$. 
Hence, $w(q_0)=1$.
Furthermore, it must be the case that 
$\sum_{(q,\psi,q')\in \eta} w(q,\psi,q')\leq |\Upsilon|\cdot w(q)$.
Indeed, for all successors $q'$ of $(q,\psi,q')$ the weight of
$(q,\psi,q')$ is induced 
by the same set of nodes $X_q$ in the tree and $X_q$ has at most
$|X_q|\cdot |\Upsilon|$  
children in $T$.
Finally, $w(q,\psi,q')\geq w(q')$ as $w(q,\psi,q')$ is chosen
according to  
the number of children of $X_q$ that are labeled by $q'$.
As $X_{q'}$ is chosen as the minimal set, it follows that
$w(q,\psi,q')\geq w(q')$. 
\end{compactitem}
\end{proof}

\begin{corollary}
In a weight distribution for $\cD$ and branching $\Upsilon$ all
weights are bounded by $|\Upsilon|^{|Q|}$.
It follows that the decision of whether the language of a transducer
$\cD$ is coverable is in NP.
\label{corollary:weight limit}
\end{corollary}

%\begin{corollary}
%The decision of whether the language of a transducer $\cD$ is
%coverable is in NP.
%\label{corollary:finite in NP}
%\end{corollary}

The proof of this corollary is included in Appendix.

We note that the tree is not restricted ``from above''.
That is, the words that are possible to write on branches of the tree
are all possible words over $\Psi^\omega$.
Thus, the issue of whether the language of $\cD$ is contained in a
nondeterministic language is bypassed.


==> intro.tex <==
\section{Introduction}
\label{section:intro}

\smallskip\noindent{\em Model-checking and realizability problem.}
The standard {\em model-checking} problem given a system $S$ and specification 
$A$, that describes the set of {\em allowed} behaviors, asks whether the 
system satisfies the specification, i.e., the system has only
allowed behaviors. 
In the linear-time approach, both $S$ and $A$ are considered as sets
of computations and the model-checking problem translates into a
language-inclusion problem $L(S)\subseteq L(A)$.
That is, does the language of $A$ contain all behaviors of $S$.
This is equivalent to checking whether $L(S)\cap
\overline{L(A)}\neq\emptyset$, where $\overline{L(A)}$ is the set of
computations {\em not} satisfying the specification.
In case the specification $A$ is given as a deterministic automaton,
its complement is easy to compute and we can use $L(\overline{A})$.
If $A$ is given as a temporal-logic formula $\varphi$, then we
construct directly an automaton for its complement $A_{\neg \varphi}$
\cite{VW94}.
Ultimately, model-checking is reduced to an emptiness
problem of an automaton.

In the case of {\em synthesis and realizability} the system is
expected to reply to every input of the environment by an output.
The question is whether the system can do this in an online fashion
(seeing one input at a time) in a way that satisfies the
specification.
That is, if $I$ is the set of inputs and $O$ the set of outputs, find
a mapping from $I^*$ to $O$ such that the interactions resulting from
interleaving an input with the mapped output satisfy the
specification \cite{PR89a}.
The solution calls for the construction of a two-player game modelling
this interaction.
If the specification $A$ is given by a deterministic automaton, we can
construct from it a perfect-information turn-based two-player game
$G_A$ such that the system (existential) player can \emph{realize}
some winning condition iff such a mapping exists.
Choices of the system player correspond to possible
outputs of the system and choice of the
environment player correspond to checking all possible inputs.
As the specification needs to be checked in multiple directions,
deterministic (or universal, c.f., \cite{KV05c}) automata are required
for the specification.

\smallskip\noindent{\em Temporal coverability.} 
Model checking covers only some of the aspects of correctness (and
analysis) of reactive systems.
One such alternative issue is that of {\em coverage}.
That is, both with respect to simulations and formal verification
whether the tests and specifications that are written sufficient.
In the case of simulation, various metrics are employed to consider
whether the testing done so far exercised enough of the system.
For example, one could check what parts of the code of the system was
exercised or circuit covered (for hardware) (c.f.,~the survey
\cite{TK01}).
This is similar to symbolic execution of software, an
approach that is used extensively for checking security of system code
\cite{BGM13,QYPK15}.

These approaches use structural properties of the system to guide
testing.
Alternative approaches call for trying to find types of behaviors
based on semantics.
For example, one can define a finite-state machine as a representation
of some important features of the system and check what parts of the
finite-state machine are exercised by tests (c.f., the reviews
\cite{TK01,HBCDDGHKKLSVWZ09}).

Formally stating a generalization of this approach would call for
checking whether each \emph{behavior} of a deterministic automaton
describing the specification is present in the language of the system.
That is, consider the dual problem of checking whether $L(A)\subseteq
L(S)$.
Starting from a temporal logic formula {\em temporal coverability}
would call for testing whether each behavior allowed by a temporal
logic formula is also allowed by a system.
Viewing the system and the specification, again, as automata, this
would call for solving the inverse language containment problem $L(A)
\subseteq L(S)$.
This time, as the system is nondeterministic (due to, e.g., inputs)
an algorithmic solution would call for its complementation, which
would clearly be intractable.

The classical approach of synthesis from linear temporal logic
specifications only checks that all behaviors of the controlled system
satisfy the specification. 
We rely on the ability of the environment to produce all inputs
to ensure that the controlled system still has enough behaviors.
We are not familiar with approaches that check whether the
synthesized system includes a minimal set of behaviors.

\smallskip\noindent{\em Motivating example~1.}
The authors of \cite{KPSBFP13} applied synthesis to find a program
that mimics certain aspects of a biological system.
This program was then used to further study the biological system and
suggest further experimental studies that could shed further light on
the behavior of this system (c.f., \cite{FPHH07,FHH11}).
Specification of the system was derived from biological experiments,
which included behaviors seen on the real live system.
One aspect of the synthesis problem was to require that only
experimentally observed behaviors of the system be seen in the
synthesized system.
However, in certain cases, the experimentally observed behavior
included several options for the ``same inputs''.
Thus, the synthesis question was generalized to also check that the
produced system includes a minimum of \emph{required} behaviors.
In this case, the authors of \cite{KPSBFP13} concentrated on behaviors
of bounded length.
The normal (bounded length) synthesis includes two quantifiers:
there \emph{exists} an implementation such that \emph{all} its
executions are correct.
Here, in order to include the required behavior an additional
quantifier was needed:
there \emph{exists} an implementation such that \emph{all} its
executions are correct and for \emph{every} required behavior there
\emph{exists} a matching computation.
We aim to generalize this approach beyond the case of a finite number
of executions of bounded length. 


\smallskip\noindent{\em Model-checking vs temporal coverability.}
As mentioned, the problems of model checking and temporal coverability
are dual.
The first, given system $S$ and specification $A$ calls for checking
$L(S)\subseteq L(A)$.
The second, calls for checking $L(A)\subseteq L(S)$.
As mentioned, while the specification can be deterministic (or easily
complementable through temporal logic) the system is inevitably
nondeterministic.
Thus, the model-checking problem is polynomial in the size of the
system.
However, the temporal coverability problem would be PSPACE-complete in
the size of the system.
This is likely to be impractical, however, the algorithmic framework
within which this problem can be tackled is clear.
The clarity of this algorithmic framework allows to approximate
temporal coverability using testing approaches as mentioned above. 

\smallskip\noindent{\em Realizability vs temporal coverability
  synthesis.}
When we come to extend this approach to realizability and synthesis
the complexity lies elsewhere.
As mentioned, for every input the system has to supply an output.
If there is no restriction on the way that outputs can follow inputs
the system is in some sense universal~--~it can produce all
computations in $(I\cdot O)^\omega$.
The problem, however, becomes in producing a set of required behaviors
\emph{simultaneously}.
That is, is the branching of the inputs sufficient to allow writing
all required outputs?

The framework of games, which is the framework providing the solution
to realizability and synthesis, is no longer appropriate.
We could try to seek inspiration from the game-theoretic solution to
the language containment problem \cite{WDHR06,RCDH07}.
Namely, given a deterministic automaton $D$ and a nondeterministic
automaton $N$ we can use
a partial-information game to show that $L(D)\subseteq L(N)$.
The player trying to refute the containment would choose the input
word and the player trying to prove/verify the containment would
choose the run of $N$ on this word.
However, if the player choosing the input word knows the nondeterministic
choices of the run they could cheat.
Essentially, changing their mind while choosing the
sequence of letters of the input word based on the
nondeterministic choices made by the verifier.
If the input producing refuter is blind to the
nondeterministic choices made by the verifier then she cannot cheat.

This framework is, intuitively, appropriate as the system can react
with every possible output to every possible input leading to
nondeterminism.
However, it would have to coordinate its nondeterministic choices to
produce all possible behaviors.
This would suggest to have an existential player choosing the mapping
from inputs to outputs, another universal player choosing the input,
and a third existential player choosing the word to be covered.
As before, the player choosing the strategy needs to be
ignorant of the actual word to be covered.
Otherwise, they would be able to direct their sequence of choices to
handle that specific word.
In the context of full-information games the existential
quantification nested within the universal quantification can be
reversed resulting in just two players.
However, in the context of partial-information the order of
quantification cannot be reversed. 
This implies that we would need the context of partial-information
multi-player games.
Unfortunately, reasoning about partial-information multi-player
games is either, in some restricted cases \cite{KV00a}, of very high
complexity or, in general, undecidable \cite{PR79} (c.f.,
\cite{MW03,FS05}). 
Hence, the framework of games does not seem to offer a solution to
temporal coverability.

\smallskip\noindent{\em Our results.}
We consider the problem of temporal coverability for synthesis when
the temporal property to cover is given by a deterministic finite
automaton.
That is, find a system $S$ of branching $I$ such that the output
language of $S$ contains a specification language $L(A)$.
The space of options of $S$, by definition, includes all possible
sequence of outputs.
So the question of whether every word in $L(A)$ can be produced by $S$
trivially holds.
The complexity, intuitively, arises from the need to coordinate
between very different input sequences that would need to produce
related outputs in order to ensure that all possible output sequences
are produced.
We show that a \emph{coverability weight} on the
structure of the automaton $A$ allows us to coordinate different
parts of the tree in this way.

We then turn to the problem of realizability solving both coverability
and adherence to specification.
That is, there is an additional correctness specification $B$ and we
have to find a system $S$ of branching $I$ such that the output
language of $S$ contains $L(A)$ and at the same time the input-output
interactions of $S$ are contained in $L(B)$.
We consider the case where $A$ is a deterministic finite automaton as
before and $B$ is a deterministic B\"uchi automaton.
Clearly, if $L(A)\not\subseteq L(B)$ the task is impossible.
As $B$ is given as a deterministic automaton the check whether
$L(A)\subseteq L(B)$ is simple.
We extend our weighting argument and combine it with a ranking function
that ensures that the correctness specification is ensured as well.
In the case of coverability with correctness, we give a precondition
that ensures that coverability with correctness is possible.

\smallskip\noindent{\em Motivating example~2.} 
In synthesis it is very natural to partition the specification to
assumptions about the behavior of the environment and guarantees of
the system. This leads to a specification of the form $a \rightarrow
g$.
However, sometimes, the system has the ability to force the
environment to falsify $a$ and void the requirement to fulfil $g$.
This problem led to much research in the commuity studying synthesis
suggesting various approachs to solve it.
For example, in \cite{KP10} the authors study in what cases
specifications cannot lead to such situations.
In \cite{EKB15} the authors suggest how to ensure that the system
cooperates with the environment.
See also, \cite{BEJK14} for a survey of different approaches to solve
this problem.
Coverability offers an alternative and very different approach to try
and solve this problem.
Consider the case of input alphabet $\{1,2\}$ and output alphabet
$\{a,b,c\}$.
Suppose that the environment assumption forces the environment to
input a $2$ after seeing the output $a$.
In addition, the environment must eventually input a 1.
For an environmnent that satisfies these assumptions, the system is
required to output an infinite number of $b$s.
Clearly, the specification is easily realizable.
However, one option for the system is to always output $a$.
This implies that the environment would never be able to input $1$ and the
system would not have to output infinitely many $b$s.
Consider the language $L=(aa\{b,c\}\{a,b,c\})^*$.
We can force the system to cover this language.
However, this langugae includes $6$ words of length four, three with the third
letter $b$ and three with the third letter $c$.
It follows, that after seeing the input $2$ twice the system would
have to output a $b$ or a $c$ thus allowing the environmnet to input
the desired $1$ and forcing the system in turn to output infinitely
many $b$s in return.
The minimal required behavior forces the
system to include enough variability in its outputs to allow the
environment to fulfil its assumptions.




